Symphony: Symmetry-Equivariant Point-Centered Spherical Harmonics for 3D Molecule Generation

We present Symphony, an $E(3)$-equivariant autoregressive generative model for 3D molecular geometries that iteratively builds a molecule from molecular fragments. Existing autoregressive models such as G-SchNet and G-SphereNet for molecules utilize rotationally invariant features to respect the 3D symmetries of molecules. In contrast, Symphony uses message-passing with higher-degree $E(3)$-equivariant features. This allows a novel representation of probability distributions via spherical harmonic signals to efficiently model the 3D geometry of molecules. We show that Symphony is able to accurately generate small molecules from the QM9 dataset, outperforming existing autoregressive models and approaching the performance of diffusion models.

==> old/old_methods.tex <==
\section{Methods}
\label{sec:methods}

\textbf{Inspiration}: We build upon existing autoregressive flows, G-SchNet \citep{gschnet,cgschnet} and G-SphereNet \citep{gspherenet}.
G-SchNet uses the SchNet framework \citep{schnet} to perform message-passing with rotationally invariant
features and compute node embeddings. A focus node is then selected as the center of a 3D grid. All of the atoms in the current fragment then vote on where to place the next atom within this grid by specifying a radial distance to the next atom.
Because of the use of only rotationally invariant features, at least three atoms are needed to be present in the current fragment to specify the exact position of the next atom without any degeneracy due to symmetry; this procedure is called \emph{triangulation}. This requires several additional tokens to break symmetry.
G-SphereNet learns a normalizing flow to perform a triangulation procedure once there are atleast $3$ atoms in $\gS^{t}$.

Their approach raises several interesting questions:
\begin{itemize}
    \item Rotationally invariant features provably cannot capture complex geometrical motifs \citep{incompleteness}.
    Recently, $E(3)$-equivariant neural networks that build higher-degree rotationally equivariant features have demonstrated improved performance on a wide range of atomistic tasks \citep{nequip,e3nn,tm23}.
    Can such features improve performance in the molecular generation task as well?
    \item G-SchNet is inefficient because the model queries all of the atoms in $\gS^{t}$ to place the next atom.
    In G-SphereNet, the choice of atoms used in the triangulation procedure can change drastically when the input is perturbed slightly. Are there simpler, smoother alternatives to triangulation?
\end{itemize}
Motivated by these questions, we present Symphony which leverages message-passing with higher-degree $E(3)$-equivariant features, together with a novel parametrization of 3D probability distributions using spherical harmonic projections.

Similar to GSchNet, our model represents the position of the next atom relative to a focus atom $f$. This allows us to factorize the distribution $\pT(\r, Z; \gS^{t})$ as: 
$$
    \sum_{f} \pT^{\text{focus}}(f; \gS^{t}) \cdot \pT^{\text{atom}}(Z | f; \gS^{t}) \cdot \pT^{\text{position}}(\r | Z, f; \gS^{t})
$$
In G-SchNet, the focus is its own separate token with 3D coordinates, which unfortunately breaks symmetry. Here, we simply choose an existing atom as the focus, allowing us to capture the true probability distribution without focusing.

% This is in contrast to several reinforcement learning (RL) approaches that have become popular for molecular generation. While reinforcement learning can optimize non-differentiable losses (such as solubility and synthesizability), such methods require orders of magnitude more data samples to learn from. Our method can be augmented with reinforcement learning methods to generate samples with specific properties; we leave this investigation as future work.

Our model can be described by the following sequence of operations, shown graphically in \autoref{fig:model_construction}.

\textbf{1. Computing Node Embeddings with Message-Passing}: As depicted in Panel 1 of \autoref{fig:model_construction}, we first compute node embeddings $h_i$ for each atom $i$ in the graph using an $E(3)$-equivariant message-passing network (here, NequIP \citep{nequip}). These node embeddings capture the geometry of every node's local neighborhood. In the interest of space, we describe how the embeddings are computed in \autoref{sec:nequip}.


\textbf{2. Predicting a Focus Node $f$}:
The prediction of the focus atom should be invariant to rotations and translations of $\gS^{t}$.
Thus, as shown in Panel 2 of  \autoref{fig:model_construction}, the scalar $l = 0$ component of these node embeddings is passed through a multi-layer perceptron (MLP) to predict a focus atom $f$ among all of the atom in $\gS^{t}$. 

\textbf{3. Predicting the Target Atomic Number $Z$}:
Similarly, the prediction of the atomic number $Z$ should be invariant to rotations and translations of $\gS^{t}$. Thus, only the scalar $l = 0$ component of the focus node's embedding $h_f$ is used by an MLP to predict the atomic number $Z$ of the next atom to be placed. This is shown in Panel 3 of \autoref{fig:model_construction}.

\textbf{4. Predicting the Target Position $\r$}: As visualized in Panels 4a and 4b of \autoref{fig:model_construction}, all of the components of the focus node's embedding $h_f$ and the provided atom type $Z$ are used to predict the position of the next atom to be placed. 

The position is represented by spherical coordinates $r, \theta, \phi$ where $r$ is the distance from the focus $f$, $\theta$ is the polar angle and $\phi$ is the azimuthal angle.
Any probability distribution $\pT$ over positions must satisfy the normalization and non-negativity constraints
$
\int_{\Omega} \pT(r, \theta, \phi) \ dV = 1$ and $
\pT(r, \theta, \phi) \geq 0
$,
where $dV = r dr \sin \theta d\theta d\phi$ is the volume element and $\Omega = \{ r \in [0, \infty),
\theta \in [0, \pi], \phi \in [0, 2\pi)\}$ represents all space in spherical coordinates.
Since these constraints are hard to incorporate directly into a neural network, we predict the logits $\fT(r, \theta, \phi)$ instead, and take the softmax over all space:
$
\pT(r, \theta, \phi) = \frac{\exp{\fT(r, \theta, \phi)}}{\int_{\Omega}\exp{\fT(r', \theta', \phi')} \ dV'}
$.
To model these logits, we
first discretize the radial component $r$ into a set of $64$ equally-spaced values from $0.75$A to $2$A covering the usual range of bond lengths in QM9 \citep{qm9}. For each fixed value of $r$, we obtain a function on the sphere $S^2$, which we represent in the basis of spherical harmonic functions $Y^l_{m}(\theta, \phi)$, as described in \autoref{sec:background}. As we have a radial component $r$ here, the coefficients $c^{(l)}$ also depend on $r$:
$\fT(r, \theta, \phi; \gS^{t}) = \sum_{l = 0}^{\infty} c^{(l)}(r; \gS^{t})^T Y^l(\theta, \phi)
$.

Our model predicts these coefficients $c^{(l)}$ upto a predefined cutoff $l_\text{max}$. In \autoref{sec:experiments}, we see the effect of varying $l_\text{max}$ upto $5$.

Note that our probability distribution $\pT$ is centered at our focus atom. 
Thus, as long as the focus prediction is invariant to translations, $\pT$ will also be invariant to translations.
To guarantee that $\pT$ is additionally $E(3)$-equivariant, we show in \autoref{sec:equivariance-proof} that the coefficients $c^{(l)}$ for every $l$ must also transform as an irreducible representation of $O(3)$ of degree $l$:
$
c^{(l)}(r; \R\gS^{t}) = D^l(\R)^T c^{(l)}(r; \gS^{t})
$.

\subsection{Learning Parameters $\Theta$}
\label{sec:training}

Following \citet{gschnet},  we split QM9 into a training set of $\approx 50,000$ molecules, a validation set of $\approx 5,000$ molecules, and a test set of $\approx 80,000$ molecules.

First, we describe how the training trajectories are created.
Given a molecule from the training set, we randomly select an atom from which to start generating fragments. This atom is marked as visited.
We randomly select a focus atom from the currently unvisited atoms that are within a set distance $d$ from the last placed atom. We then randomly select the next atom from the atoms within $d$ of our current focus atom. This target atom is included as part of the generated fragment, and we repeat this process until all atoms in the molecule have been visited.
This gives us a training trajectory for the molecule. We create many such trajectories corresponding to different choices of focus atoms at each step.

Similar to existing autoregressive models, we use \emph{teacher-forcing} to train the model. We generate training trajectories by breaking down molecules into several sequences of placement steps, providing supervision for the correct focus, atom type and position at every step: 

\begin{itemize}
\item 
\textbf{Predicting a Focus Node $f$}:
For each graph, we compute:
$$
L_{\text{focus}} = -\sum_{v \in V} q_v \cdot f_v + \log\left(1 + \sum_{v \in V} \exp(f_v)\right)
$$
where $q_v$ is the probability of the focus atom being node $v$, $f_v$ is the output of our focus MLP at $v$, and $V$ is the set of all atoms in the graph.

\item \textbf{Predicting the Target Atomic Number $Z$}:
We compute the standard cross-entropy loss between the predicted target atom type distribution and the actual target atom type.

\item \textbf{Predicting the Target Position $\r$}:
We define the target distribution $q$ as a Dirac delta distribution centered at the true position $\r_{n + 1}$ of the next atom to be placed, according to our training trajectory.

For a given target distance distribution $q$ and predicted distribution $p_{\Theta}$, the KL divergence is defined as follows:
$$L_{\text{position}} = \infdiv{q}{p_{\Theta}} = \int_{\Omega} q(r, \theta, \phi) \log \frac{q(r, \theta, \phi)}{p_{\Theta}(r, \theta, \phi)} \, dV$$
\end{itemize}

Our loss is $
L_\text{total} = L_{\text{focus}} + L_{\text{atom-type}} + L_{\text{position}}
$. Since our loss is completely differentiable, we optimize our parameters with the Adam \citep{adam} optimizer, a variant of stochastic gradient descent, with a learning rate of $10^{-3}$ and a batch size of $16$ graphs.

We also add a small amount of Gaussian noise sampled from $\mathcal{N}(\mu = 0, \sigma = 0.05A)$ to the true atomic positions at every step. This helps performance at inference time when the model's errors may potentially accumulate due to recursively chaining model predictions over multiple generation steps.

\subsection{Building Molecules}
Once we have learned our parameters $\Theta$, we can iteratively sample from the learned distributions to generate entire molecules, as shown in \autoref{fig:model_construction}.

We initialize with $\gS^{1} = \{([0, 0, 0], \text{H})\}$, representing a single hydrogen atom at the origin.
We repeat the following steps until a STOP is predicted:
\begin{itemize}
    \item We predict a focus atom $f$ by sampling from $\pT^{\text{focus}}(\cdot; \gS^{t})$. The spherical harmonic projections are centered at the focus atom $f$.
    If STOP was predicted, end sampling and return $\gS^{t}$.
    \item We predict an atom type $Z_{n + 1}$ by sampling from $\pT^{\text{atom}}(\cdot \ | \ f; \gS^{t})$.
    \item We predict the position $\r_{n + 1}$ by sampling from $\pT^{\text{position}}(\cdot \ | \ f, Z; \gS^{t})$.
    \item We add $Z_{n + 1}$ and $\r_{n + 1}$ to $\gS^{t}$, giving us $\gS^{t + 1}$.
\end{itemize}


We control the creativity of our model by temperature sampling \cite{calibration}, i.e. multiplying the logits of each of the predicted distributions by an inverse temperature parameter $\beta$. Increasing $\beta$ makes the distributions more peaked, while lowering $\beta$ makes the distribution more uniform.

Finally, since many molecular generation metrics require bonding information, we use the \texttt{xyz2mol} \citep{xyz2mol} package in RDKit \citep{rdkit} to infer bonding orders given 3D atomic positions.

==> old/old_model_details.tex <==
\section{Details on Symphony}
\textbf{1. Computing Node Embeddings with Message-Passing}: As depicted in Panel 1 of \autoref{fig:model_construction}, we first compute node embeddings $h_i$ for each atom $i$ in the graph using an $E(3)$-equivariant message-passing network (here, NequIP \citep{nequip}). These node embeddings capture the geometry of every node's local neighborhood. In the interest of space, we describe how the embeddings are computed in \autoref{sec:nequip}.


\textbf{2. Predicting a Focus Node $f$}:
The prediction of the focus atom should be invariant to rotations and translations of $\gS^n$.
Thus, as shown in Panel 2 of  \autoref{fig:model_construction}, the scalar $l = 0$ component of these node embeddings is passed through a multi-layer perceptron (MLP) to predict a focus atom $f$ among all of the atom in $\gS^{n}$. 

\textbf{3. Predicting the Target Atomic Number $Z$}:
Similarly, the prediction of the atomic number $Z$ should be invariant to rotations and translations of $\gS^n$. Thus, only the scalar $l = 0$ component of the focus node's embedding $h_f$ is used by an MLP to predict the atomic number $Z$ of the next atom to be placed. This is shown in Panel 3 of \autoref{fig:model_construction}.

\textbf{4. Predicting the Target Position $\r$}: As visualized in Panels 4a and 4b of \autoref{fig:model_construction}, all of the components of the focus node's embedding $h_f$ and the provided atom type $Z$ are used to predict the position of the next atom to be placed. '

